Comix, a new matrix element generator

We present a new tree-level matrix element generator, based on the colour dressed Berends-Giele recursive relations. We discuss two new algorithms for phase space integration, dedicated to be used with large multiplicities and colour sampling.

==> text/lorentz.tex <==
In this appendix we list explicit expressions for all possible Lorentz 
vertex structures occuring in the Berends-Giele recursion defined by the 
Standard Model. We sort them by ascending spin of the connecting particles
and employ the following notation.\\[1.5ex]
\begin{tabular}{cl}
S &Scalar,\\
F &Fermion,\\
V &Vector Boson,\\
T &Antisymmetric tensor of rank two.
\end{tabular}\\[2ex]
We stress again that all interaction terms occuring in the Standard Model
Lagrangian yield no more than three-particle vertices of the above defined
particle types with the possible couplings listed in Appendix~\ref{sec:vertex}.
The quantities listed in Tab.~\ref{tab:lorentz_types} in explicit form
are given by
\begin{align}\label{eq:cpl_ffvr_a}
  \bar{u}j^\mu\gamma_\mu \frac{1-\gamma^5}{2} 
    &=\rbr{0,0,\bar{u}_0j^--\bar{u}_1j_\perp,
    -\bar{u}_0j_\perp^*+\bar{u}_1j^+}\;,
\end{align}
\begin{align}\label{eq:cpl_ffvr_b}
  j^\mu\gamma_\mu \frac{1-\gamma^5}{2} v
    &=\left(\begin{array}{c}0\\0\\
     j^+v_0+j_\perp^*v_1\\j_\perp v_0+j^-v_1\end{array}\right)\;,
  &\bar{u}\gamma^\mu \frac{1-\gamma^5}{2} v 
    &=\left(\begin{array}{c}
      \bar{u}_0v_2+\bar{u}_1v_3\\
      \bar{u}_0v_3+\bar{u}_1v_2\\
      i\left(\bar{u}_1v_2-\bar{u}_0v_3\right)\\
      \bar{u}_0v_2-\bar{u}_1v_3\end{array}\right)\;,
\end{align}
\begin{align}\label{eq:cpl_ffvl_a}
  \bar{u}j^\mu\gamma_\mu \frac{1+\gamma^5}{2}
    &=\rbr{\bar{u}_2j^++\bar{u}_3j_\perp,
    \bar{u}_2j_\perp^*+\bar{u}_3j^-,0,0}\;,
\end{align}
\begin{align}\label{eq:cpl_ffvl_b}
  j^\mu\gamma_\mu \frac{1+\gamma^5}{2} v
    &=\left(\begin{array}{c}
    j^-v_2-j_\perp^*v_3\\-j_\perp v_2+j^+v_3\\
    0\\0\end{array}\right)\;,
  &\bar{u}\gamma^\mu \frac{1+\gamma^5}{2} v
    &=\left(\begin{array}{c}
    \bar{u}_2v_0+\bar{u}_3v_1\\
    -\bar{u}_2v_1-\bar{u}_3v_0\\
    i\left(\bar{u}_2v_1-\bar{u}_3v_0\right)\\
    -\bar{u}_2v_0+\bar{u}_3v_1\end{array}\right)\;,
\end{align}
\begin{align}
  \Gamma^{\nu\lambda\kappa}\rbr{p,q}\varepsilon_\lambda\varepsilon'_\kappa
    &=\varepsilon\varepsilon'\rbr{p-q}^\nu
    +\varepsilon'\rbr{2q+p}\varepsilon^\nu
    -\varepsilon\rbr{2p+q}\varepsilon'^\nu\;,
\end{align}
\begin{align}
  \tau^{\mu\nu}\rbr{\varepsilon,\varepsilon'}
    &=\frac{1}{2}\rbr{g^{\mu\lambda}g^{\nu\kappa}-g^{\mu\kappa}g^{\nu\lambda}}
      \varepsilon_\lambda\varepsilon'_\kappa\;.
\end{align}
Note that due to the antisymmetry of $\tau^{\mu\nu}$, we can make
the replacement
\begin{equation}
  \frac{1}{2}\rbr{g^\mu_\alpha g^\nu_\beta-g^\mu_\beta g^\nu_\alpha}
    \tau^{\alpha\beta}
    =\tau^{\mu\nu}
\end{equation} 
which leads to an asymmetric form of the VVT vertex, and a slight
decrease in evaluation time.\clearpage
\mytable{h!}{
  \begin{tabular}{|c|>{\centering}p{3cm}>{\centering}p{3cm}>{\centering}p{3cm}@{}l|}
    \hline & & & &\\
    \large\bf Vertex ID & 
    \multicolumn{4}{c|}{\large\bf Lorentz structures}\\ 
    & & & &\\\hline& & & &\\[-1em]
    FFS & \vxxs{fermion}{plain}{\bar u}{v} 
    & \vxxr{fermion}{plain}{s}{v}      
    & \vxxl{fermion}{plain}{\bar u}{s} & \\
    & $\dst\bar{u}\,v$ & $\dst s\,v$ & $\dst\bar{u}\,s$ &\\[3mm]\hline& & & &\\[-1em]
    FFV$^-$ & \vxxs{fermion}{photon}{\bar u}{v}
    & \vxxr{fermion}{photon}{\varepsilon}{v}
    & \vxxl{fermion}{photon}{\bar u}{\varepsilon} & \\
    & $\dst\bar{u}\gamma^\mu \frac{1-\gamma^5}{2} v$ &
    $\dst\varepsilon^\mu\gamma_\mu \frac{1-\gamma^5}{2} v$ &
    $\dst\bar{u}\varepsilon^\mu\gamma_\mu \frac{1-\gamma^5}{2}$ &\\[3mm]\hline& & & &\\[-1em]
    FFV$^+$ & \vxxs{fermion}{photon}{\bar u}{v}
    & \vxxr{fermion}{photon}{\varepsilon}{v}
    & \vxxl{fermion}{photon}{\bar u}{\varepsilon} & \\
    & $\dst\bar{u}\gamma^\mu \frac{1+\gamma^5}{2} v$ &
    $\dst\varepsilon^\mu\gamma_\mu \frac{1+\gamma^5}{2} v$ &
    $\dst\bar{u}\varepsilon^\mu\gamma_\mu \frac{1+\gamma^5}{2}$ &\\[3mm]\hline& & & &\\[-1em]
    VVS & \vxxs{photon}{dashes}{\varepsilon}{\varepsilon'}
    & \vxxr{photon}{dashes}{s}{\varepsilon'} & & \\
    & $\dst\varepsilon^\mu\varepsilon'_\mu$ &
    $\dst s\,\varepsilon'^\mu$ & &\\[3mm]\hline& & & &\\[-0.5em]
    VVV$\rbr{p,q}$ & \vxxs{photon}{photon}{\varepsilon(p)}{\varepsilon'(q)} & & &\\
    & $\dst\Gamma^{\nu\lambda\kappa}\rbr{p,q}\varepsilon_\lambda\varepsilon'_\kappa$ & & &\\[3mm]
    \hline& & & &\\[-0.5em]
    VVT & \vxxs{photon}{dots}{\varepsilon}{\varepsilon'}
    & \vxxl{photon}{dots}{\varepsilon}{\tau} &{\hfill} &\\
    & $\dst\tau^{\mu\nu}\rbr{\varepsilon,\varepsilon'}$ &
    $\dst\varepsilon_\nu\tau^{\mu\nu}$ & &\\[-0.5em]
    & & & &\\\hline
  \end{tabular}\vspace*{2ex}
  }{Lorentz structures of Standard Model interactions.
    \label{tab:lorentz_types}}


==> text/vertex.tex <==
In this appendix we explicitly list all vertices occuring in the
recursive relations for the Standard Model as formulated in Sec.~\ref{sec:sm}.
Their Lorentz structures are defined in Appendix~\ref{sec:lorentz}.
\begin{longtable}{c@{\hspace{1ex}=\hspace{3ex}}l@{\hspace{2ex}}}
  \multicolumn{2}{c}{\large\bf QCD interactions}\\
  \ixxs{fermion}{gluon}{q,,K}{\bar q,,\bar L}{g,,H\bar G} & 
  $\dst -i\,\frac{g_s}{\sqrt{2}}\,\sbr{\;\delta_H^K\delta_{\bar G}^{\bar L}
     -\frac{1}{N_C}\delta_{H\bar G}\delta^{K\bar L}\,}\,
     \rbr{\;{\rm FFV}^-+{\rm FFV}^+\,}$ \\
  \ixxf{gluon}{gluon}{g(p),,K\bar L}{g(q),,M\bar N}{g,,H\bar G} & 
  $\dst i\,\frac{g_s}{\sqrt{2}}\,\sbr{\;
     \delta_H^M\delta^{K\bar N}\delta_{\bar G}^{\bar L}\;{\rm VVV}\rbr{p,q}
     -\delta_H^K\delta^{\bar L M}\delta_{\bar G}^{\bar N}\;
     {\rm VVV}\rbr{q,p}\;}$ \\
  \ixxf{gluon}{dots}{g,,K\bar L}{g,,M\bar N}{g_4,,H\bar G} & 
  $\dst i\,\frac{g_s}{\sqrt{2}}\,\sbr{\;
     \delta_H^K\delta^{\bar L M}\delta_{\bar G}^{\bar N}
     -\delta_H^M\delta^{K\bar N}\delta_{\bar G}^{\bar L}\;}\;{\rm VVT}$ \\
  \prpr{quark}{q}{H}{I} & 
  $\dst i\,\delta_I^H\,\frac{\hat p+m}{p^2-m^2}$ \\
  \prpr{gluon}{g}{\nu,,H\bar G}{\mu,,I\bar J} & 
  $\dst i\,\delta_I^H\delta_{\bar J}^{\bar G}\,\frac{-g_{\mu\nu}}{p^2}$ \\
  \prpr{dots}{g_4}{\mu\nu,,H\bar G}{\rho\sigma,,I\bar J} & 
  $\dst -i\,\delta_I^H\delta_{\bar J}^{\bar G}\,D_{\mu\nu}^{\rho\sigma}$ \\
  \multicolumn{2}{c}{\large\bf QED interactions}\\
  \ixxs{fermion}{photon}{f}{\bar f}{\gamma} & 
  $\dst -i\,g_eQ_f\,\rbr{\;{\rm FFV}^-+{\rm FFV}^+\,}$ \\
  \prpr{fermion}{f}{}{} & 
  $\dst i\,\frac{\hat p+m_f}{p^2-m_f^2}$ \\
  \prpr{photon}{\gamma}{\nu}{\mu} & 
  $\dst i\,\frac{-g_{\mu\nu}+p^\mu p^\nu/p^2}{p^2}$ \\
  \multicolumn{2}{c}{\large\bf Electroweak interactions}\\
  \ixxs{dashes}{dashes}{h}{h}{h} & 
  $\dst i\,\frac{3\,m_h^2}{v}$ \\
  \ixxs{dashes}{dashes}{h}{h}{h_4} & 
  $\dst i\,\frac{m_h^2}{v^2}$ \hspace*{1cm}
  \ixxs{dashes}{dashes}{h}{h_4}{h}\hspace*{1ex}=\hspace*{3ex}
  $\dst i$ \\
  \ixxs{fermion}{dashes}{f}{\bar f}{h} & 
  $\dst -i\,\frac{m_f}{v}\;{\rm FFS}$ \\
  \ixxs{fermion}{wiggly}{f}{\bar f}{Z} & 
  $\dst -i\,\frac{g_w}{2\cos\theta_W}\,
     \cbr{\;\rbr{V_f+A_f}{\rm FFV}^-+\rbr{V_f-A_f}{\rm FFV}^+\,}$ \\
  \ixxs{fermion}{wiggly}{f}{\bar f'}{W^+} & 
  $\dst -i\,\frac{g_w}{\sqrt{2}}\;T_{ff'}^+\;{\rm FFV}^-$ \\
  \ixxs{wiggly}{dashes}{W/Z}{W/Z}{h} & 
  $\dst -i\,\frac{g_w\,m_{W/Z}}{\lambda_{W/Z}}\,VVS
    \quad\quad{\rm where}\quad\quad
    \begin{array}{rc}\lambda_W\,=&1\\
      \lambda_Z\,=&\cos\theta_W\end{array}$ \\
  \ixxs{wiggly}{dashes}{W/Z}{W/Z}{h_4} & 
  $\dst -i\,\frac{g_w^2}{2\,\lambda_{W/Z}^2}\,VVS
    \quad\quad{\rm where}\quad\quad\begin{array}{rc}\lambda_W\,=&1\\
      \lambda_Z\,=&\cos\theta_W\end{array}$ \\
  \ixxs{wiggly}{wiggly}{W^-(p)}{W^+(q)}{A/Z} & 
  $\dst i\,g_w\,\kappa_{A/Z}\,VVV\rbr{p,q}\quad\quad{\rm where}\quad\quad
    \begin{array}{rl}\kappa_A&=\,\sin\theta_W\\
      \kappa_Z&=\,\cos\theta_W\end{array}$ \\
  \ixxs{wiggly}{dots}{W^-}{W^+}{Z_4} & 
  $\dst i\,g_w\,VVT$ \\
  \ixxs{wiggly}{dots}{W^-}{A/Z}{W_4^-} & 
  $\dst i\,g_w\,\kappa_{A/Z}\,VVT\quad\quad{\rm where}\quad\quad
    \begin{array}{rl}\kappa_A&=\,\sin\theta_W\\
      \kappa_Z&=\,\cos\theta_W\end{array}$ \\
  \prpr{dashes}{h}{}{} & 
  $\dst \frac{i}{p^2-m_h^2}$ \hspace*{1cm}
  \prpr{dashes}{h_4}{}{}\hspace*{1ex}=\hspace*{3ex}
  $\dst i$ \\
  \prpr{wiggly}{W/Z}{\nu}{\mu} & 
  $\dst i\,\frac{-g_{\mu\nu}+p^\mu p^\nu/m_{W/Z}^2}{p^2-m_{W/Z}^2}$ \\
  \prpr{dots}{Z_4}{\rho\sigma}{\mu\nu} & 
  $\dst -i\,D_{\mu\nu}^{\,\rho\sigma}$ \hspace*{1cm}
  \prpr{dots}{W_4^\pm}{\rho\sigma}{\mu\nu}\hspace*{1ex}=\hspace*{3ex}
  $\dst i\,D_{\mu\nu}^{\,\rho\sigma}$ \\
\end{longtable}
Here we have defined
\begin{align*}
  V_f&=T_f^3-2Q_f\sin^2\theta_W,&A_f&=T_f^3\;.
\end{align*}

